PEMS: Pre-trained Epidemic Time-series Models

Providing accurate and reliable predictions about the future of an epidemic is an important problem for enabling informed public health decisions. Recent works have shown that leveraging data-driven solutions that utilize advances in deep learning methods to learn from past data of an epidemic often outperform traditional mechanistic models. However, in many cases, the past data is sparse and may not sufficiently capture the underlying dynamics. While there exists a large amount of data from past epidemics, leveraging prior knowledge from time-series data of other diseases is a non-trivial challenge. Motivated by the success of pre-trained models in language and vision tasks, we tackle the problem of pre-training epidemic time-series models to learn from multiple datasets from different diseases and epidemics. We introduce Pre-trained Epidemic Time-Series Models (PEMS) that learn from diverse time-series datasets of a variety of diseases by formulating pre-training as a set of self-supervised learning (SSL) tasks. We tackle various important challenges specific to pre-training for epidemic time-series such as dealing with heterogeneous dynamics and efficiently capturing useful patterns from multiple epidemic datasets by carefully designing the SSL tasks to learn important priors about the epidemic dynamics that can be leveraged for fine-tuning to multiple downstream tasks. The resultant PEM outperforms previous state-of-the-art methods in various downstream time-series tasks across datasets of varying seasonal patterns, geography, and mechanism of contagion including the novel Covid-19 pandemic unseen in pre-trained data with better efficiency using smaller fraction of datasets.

==> Text/related_short.tex <==
\section{Related works}
\paragraph{Neural models for time-series analysis}
%Deep neural networks have been widely used in many time series forecasting
%applications with great success.
Popular deep-learning time-series models include auto-regressive recurrent networks~\cite{salinas2020deepar},
Deep Markov models \cite{krishnan2017structured} and Deep State Space models \cite{rangapuram2018deep, li2021learning, gu2021efficiently}.
Recent works leveraged and extended transformers to better capture long-term 
trends resulting in state-of-art performance~\cite{zhou2021informer,chen2021autoformer,zhou2022fedformer,liu2021pyraformer}.
However, all these methods do not leverage pre-training and can not learn from multiple heterogenous pre-train datasets that are not in training data.
%They follow the typical supervised learning paradigm of
%leveraging training data from past values of the same dataset to
%forecast future values.% and do not leverage cross-domain heterogenous
%%datasets or aim to provide generalized models that can be used for a wide range of
%heterogeneous tasks.


\paragraph{Self-supervised learning for time-series}
Recent works have shown the efficacy of
self-supervised representation learning for time-series for various classification
and forecasting tasks~\cite{merrill2022self,chowdhury2022tarnet,zhang2019deep,zhang2022self,franceschi2019unsupervised}.
They leverage similarities of time-series in datasets by leveraging contrastive learning~\cite{eldele2021time,yue2022ts2vec} and other time-series similarity metrics~\cite{tonekaboni2021unsupervised,franceschi2019unsupervised} to train on unlabeled time-series datasets.
However, all these methods apply SSL on the same dataset that is used for training and may not adapt well to using time-series multiple sources
such as time-series from multiple diseases.
%Our work, in contrast, tackles the problem of learning general models
%from a wide range of heterogenous datasets that can be fine-tuned
%%for a wide variety of tasks on multiple datasets that may not be
%seen during pre-training.
%Therefore, we design SSL tasks that can adapt to multiple time-series datasets and capture useful underlying properties from
%these datasets for superior performance on multiple downstream applications on various disease forecasting tasks.

\paragraph{Statistical models for epidemic forecasting}
%Due to recent advances in machine learning and deep learning as well as the availability of datasets from various surveillance
%sources, statistical and deep-learning-based models are increasingly used for epidemic forecasting tasks with great success~\cite{rodriguez2022data}.
Classical auto-regressive time-series models like ARIMA and its variants
have been adapted for disease forecasting~\cite{soebiyanto2010modeling,yang2015accurate}.
Other models use probabilistic  approaches~\cite{brooks2015flexible,brooks2018nonmechanistic,zimmer2020influenza}
 have been successful in past epidemic forecasting competitions~\cite{reich_collaborative_2019}.% like
%Flusight~\cite{reich_collaborative_2019}.
%Other classical machine-learning methods like Gaussian Processes~\cite{zimmer2020influenza},
%Generalized Linear models~\cite{chakraborty_what_2018} and nearest-neighbor-based regression~\cite{chakraborty2014forecasting} have also been adapted.
Recent works increasingly use deep learning methods such as
recurrent neural models~\cite{venna2018novel}.  Other works exploit
important characteristics of epidemic dynamics such as dynamically modeling sequence similarity across seasons~\cite{adhikari2019epideep,kamarthi2021doubt}, exploiting spatial relations~\cite{deng2020cola,kamarthi2022camul} across regions
as well as use expert priors such as traditional mechanistic models~\cite{rodriguez2022einns,Gao2021STANSA}.
However, most previous works train only from past data for epidemics they forecast and do not leverage useful background
knowledge from a large amount of epidemic data of other diseases collected in the past.
